Analyzing the Impact of Elusive Faults on Blockchain Reliability

Blockchain recently became very popular due to its use in cryptocurrencies and potential application in various domains (e.g., retail, healthcare, insurance). The smart contract is a key part of blockchain systems and specifies an agreement between transaction participants. Nowadays, smart contracts are being deployed carrying residual faults, including severe vulnerabilities that lead to different types of failures at runtime. Fault detection tools can be used to detect faults that may then be removed from the code before deployment. However, in the case of smart contracts, the common opinion is that tools are immature and ineffective. In this work, we carry out a fault injection campaign to empirically analyze the runtime impact that realistic faults present in smart contracts may have on the reliability of blockchain systems. We place particular attention on the faults that elude popular smart contract verification tools and show if and in which ways the faults lead the blockchain system to fail at runtime. Results show general poor detection and, to some extent, complementary performance by the three tools used. The results also show that several elusive faults are responsible for severe blockchain failures.

==> tables/fault-model-2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{}
\label{tab:my-table}
\begin{tabular}{|l|c|l|l|l|}
\hline
   & \multicolumn{1}{l|}{\textbf{Defect Class}} & \textbf{Defect Nature}   & \textbf{Defect Name}                                                                  & \textbf{Defect   Identifier} \\ \hline
1  & {Assignment}               & {Missing} & Initialization of Storage Variables/Pointers (Uninitialized Storage Pointer)   (MISP) & A\_MISP                       \\ \cline{1-1} \cline{4-5} 
2  &                                            &                          & Initialization of Local Variable (MILV)                                               & A\_MILV                       \\ \cline{1-1} \cline{4-5} 
3  &                                            &                          & Initialization of State Variables (MISV)                                              & A\_MISV                       \\ \cline{1-1} \cline{4-5} 
4  &                                            &                          & Constructor (MC)                                                                      & A\_MC                         \\ \cline{1-1} \cline{4-5} 
5  &                                            &                          & Compiler Version (MCV)                                                                & A\_MCV                        \\ \cline{1-1} \cline{3-5} 
6  &                                            & {Wrong}   & Arithmetic Expression Used In Assignment (WVAE)                                       & A\_WVAE                       \\ \cline{1-1} \cline{4-5} 
7  &                                            &                          & Integer Sign (WIS)                                                                    & A\_WIS                        \\ \cline{1-1} \cline{4-5} 
8  &                                            &                          & Integer Truncation (WIT)                                                              & A\_WIT                        \\ \cline{1-1} \cline{4-5} 
9  &                                            &                          & Value Assignment With Too Many Digits (WVATMD)                                        & A\_WVATMD                     \\ \cline{1-1} \cline{4-5} 
10 &                                            &                          & Value Assigned To Contract Address (WVAA)                                             & A\_WVAA                       \\ \cline{1-1} \cline{4-5} 
11 &                                            &                          & Constructor Name (WCN)                                                                & A\_WCN                        \\ \cline{1-1} \cline{4-5} 
12 &                                            &                          & Variable Type (e.g., byte[]) (WVT)                                                    & A\_WVT                        \\ \cline{1-1} \cline{4-5} 
13 &                                            &                          & Declaration Of Invariant State Variable (WDISV)                                       & A\_WDISV                      \\ \cline{1-1} \cline{4-5} 
14 &                                            &                          & Variable Name (Variable Shadowing) (WVN)                                              & A\_WVN                        \\ \hline
15 & {Checking}                 & {Missing} & "require" On Transaction Sender (MRTS)                                                & CH_MRTS                      \\ \cline{1-1} \cline{4-5} 
16 &                                            &                          & "require" On Input Variable(s) (MRIV)                                                 & CH_MRIV                      \\ \cline{1-1} \cline{4-5} 
17 &                                            &                          & "require" OR Subexpression On Transaction Sender (MROTS)                              & CH_MROTS                     \\ \cline{1-1} \cline{4-5} 
18 &                                            &                          & "require" OR Subexpression On Input Variable(s) (MROIV)                               & CH_MROIV                     \\ \cline{1-1} \cline{4-5} 
19 &                                            &                          & "require" AND Subexpression On Transaction Sender (MRATS)                             & CH_MRATS                     \\ \cline{1-1} \cline{4-5} 
20 &                                            &                          & "require" AND Subexpression On Input Variable(s) (MRAIV)                              & CH_MRAIV                     \\ \cline{1-1} \cline{4-5} 
21 &                                            &                          & Check On Gas Limit (MCHGL)                                                            & CH_MCHGL                     \\ \cline{1-1} \cline{4-5} 
22 &                                            &                          & Check On Arithmetic Operation (MCHAO)                                                 & CH_MCHAO                     \\ \cline{1-1} \cline{4-5} 
23 &                                            &                          & Check On Suicide Functionality (MCHSF)                                                & CH_MCHSF                     \\ \cline{1-1} \cline{3-5} 
24 &                                            & Wrong                    & "require" For Authorization (Authorization Through tx.origin) (WRA)                   & CH_WRA                       \\ \hline
25 & {Interface}                 & {Missing} & Visibility modifier of state variables (implicit visibility) (MVMSV)                  & I\_MVMSV                      \\ \cline{1-1} \cline{4-5} 
26 &                                            &                          & Function Visibility Modifier (MFVM)                                                   & I\_MFVM                       \\ \cline{1-1} \cline{3-5} 
27 &                                            & Wrong                    & visibility (public) for private/internal function (WVPF)                              & I\_WVPF                       \\ \hline
28 & {Algorithm}                 & {Missing} & "if" construct on transaction sender plus statements (MITSS)                          & AL_MITSS                     \\ \cline{1-1} \cline{4-5} 
29 &                                            &                          & "if" construct on input variable(s) plus statements (MIIVS)                           & AL_MIIVS                     \\ \cline{1-1} \cline{3-5} 
30 &                                            & {Wrong}   & use of require, assert, and revert (WRAR)                                             & AL_WRAR                      \\ \cline{1-1} \cline{4-5} 
31 &                                            &                          & Exception Handling (WEH)                                                              & AL_WEH                       \\ \cline{1-1} \cline{3-5} 
32 &                                            & Extraneous               & continue-statements in do-while-statements or for (ECSWS)                             & AL_ECSWS                     \\ \hline
33 & {Function}                  & {Missing} & Withdraw function (MWF)                                                               & F_MWF                        \\ \cline{1-1} \cline{4-5} 
34 &                                            &                          & Inheritance (MINHERITANCE)                                                            & F_MINHERITANCE               \\ \cline{1-1} \cline{3-5} 
35 &                                            & Wrong                    & Inheritance and inheritance Order (WIO)                                               & F_WIO                        \\ \cline{1-1} \cline{3-5} 
36 &                                            & Extraneous               & Inheritance (EINHERITANCE)                                                            & F_EINHERITANCE               \\ \hline
\end{tabular}
\end{table}

==> tables/fault-model.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\renewcommand{\arraystretch}{1.2}
\begin{table}[ht]
\caption{Smart contract defect classification \cite{prdc2021}}
\label{tab:scheme}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Defect   Class}      & \textbf{Defect Nature}   & \textbf{Defect Name}                                                                  & \textbf{Defect   Identifier} \\
\hline \hline
{Assignment} & {Missing} & Initialization of Storage Variables/Pointers (Uninitialized Storage Pointer)   \textbf{(MISP)} & A\_MISP                       \\ \cline{3-4} 
                             &                          & Initialization of Local Variable \textbf{(MILV)}                                               & A\_MILV                       \\ \cline{3-4} 
                             &                          & Initialization of State Variables \textbf{(MISV)}                                              & A\_MISV                       \\ \cline{3-4} 
                             &                          & Constructor \textbf{(MC)}                                                                      & A\_MC                         \\ \cline{3-4} 
                             &                          & Compiler Version \textbf{(MCV)}                                                                & A\_MCV                        \\ \cline{2-4} 
                             & {Wrong}   & Arithmetic Expression Used In Assignment \textbf{(WVAE)}                                       & A\_WVAE                       \\ \cline{3-4} 
                             &                          & Integer Sign \textbf{(WIS)}                                                                    & A\_WIS                        \\ \cline{3-4} 
                             &                          & Integer Truncation \textbf{(WIT)}                                                              & A\_WIT                        \\ \cline{3-4} 
                             &                          & Value Assignment With Too Many Digits \textbf{(WVATMD)}                                        & A\_WVATMD                     \\ \cline{3-4} 
                             &                          & Value Assigned To Contract Address \textbf{(WVAA)}                                             & A\_WVAA                       \\ \cline{3-4} 
                             &                          & Constructor Name \textbf{(WCN)}                                                                & A\_WCN                        \\ \cline{3-4} 
                             &                          & Variable Type (e.g., byte[]) \textbf{(WVT)}                                                    & A\_WVT                        \\ \cline{3-4} 
                             &                          & Declaration Of Invariant State Variable \textbf{(WDISV)}                                       & A\_WDISV                      \\ \cline{3-4} 
                             &                          & Variable Name (Variable Shadowing) \textbf{(WVN)}                                              & A\_WVN                        \\ \hline
{Checking}   & {Missing} & "require" On Transaction Sender \textbf{(MRTS)}                                                & CH\_MRTS                      \\ \cline{3-4} 
                             &                          & "require" On Input Variable(s) \textbf{(MRIV)}                                                 & CH\_MRIV                      \\ \cline{3-4} 
                             &                          & "require" OR Subexpression On Transaction Sender \textbf{(MROTS)}                              & CH\_MROTS                     \\ \cline{3-4} 
                             &                          & "require" OR Subexpression On Input Variable(s) \textbf{(MROIV)}                               & CH\_MROIV                     \\ \cline{3-4} 
                             &                          & "require" AND Subexpression On Transaction Sender \textbf{(MRATS)}                             & CH\_MRATS                     \\ \cline{3-4} 
                             &                          & "require" AND Subexpression On Input Variable(s) \textbf{(MRAIV)}                              & CH\_MRAIV                     \\ \cline{3-4} 
                             &                          & Check On Gas Limit \textbf{(MCHGL)}                                                            & CH\_MCHGL                     \\ \cline{3-4} 
                             &                          & Check On Arithmetic Operation \textbf{(MCHAO)}                                                 & CH\_MCHAO                     \\ \cline{3-4} 
                             &                          & Check On Suicide Functionality \textbf{(MCHSF)}                                                & CH\_MCHSF                     \\ \cline{2-4} 
                             & Wrong                    & "require" For Authorization (Authorization Through tx.origin) \textbf{(WRA)}                   & CH\_WRA                       \\ \hline
{Interface}   & {Missing} & Visibility modifier of state variables (implicit visibility) \textbf{(MVMSV)}                  & I\_MVMSV                      \\ \cline{3-4} 
                             &                          & Function Visibility Modifier \textbf{(MFVM)}                                                   & I\_MFVM                       \\ \cline{2-4} 
                             & Wrong                    & Visibility (public) for private/internal function \textbf{(WVPF)}                              & I\_WVPF                       \\ \hline
{Algorithm}   & {Missing} & "if" construct on transaction sender plus statements \textbf{(MITSS)}                          & AL\_MITSS                     \\ \cline{3-4} 
                             &                          & "if" construct on input variable(s) plus statements \textbf{(MIIVS)}                           & AL\_MIIVS                     \\ \cline{2-4} 
                             & {Wrong}   & Use of require, assert, and revert \textbf{(WRAR)}                                             & AL\_WRAR                      \\ \cline{3-4} 
                             &                          & Exception Handling \textbf{(WEH)}                                                              & AL\_WEH                       \\ \cline{2-4} 
                             & Extraneous               & Continue-statements in do-while-statements or for \textbf{(ECSWS)}                             & AL\_ECSWS                     \\ \hline
 {Function}    & {Missing} & Withdraw function \textbf{(MWF)}                                                               & F\_MWF                        \\ \cline{3-4} 
                             &                          & Inheritance \textbf{(MINHERITANCE)}                                                            & F\_MINHERITANCE               \\ \cline{2-4} 
                             & Wrong                    & Inheritance and inheritance Order \textbf{(WIO)}                                               & F\_WIO                        \\ \cline{2-4} 
                             & Extraneous               & Inheritance \textbf{(EINHERITANCE)}                                                            & F\_EINHERITANCE               \\ \hline
\end{tabular}
}
\end{table}

==> tables/faultGroup.tex <==
\begin{table}[h]
\centering
%\scriptsize
\caption{Failure modes and its characteristics}
\label{table:analysis-failures}
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Failure Modes}     & \textbf{\begin{tabular}[c]{@{}l@{}}Transaction \\ not concluded\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Incorrect \\ return value or \\ transaction result\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Incorrect \\ ledger state\end{tabular}} \\ \hline \hline
Abort            & \multicolumn{1}{c|}{\tiny\faCircle}                                                        &                                                                                                       &                                                                            \\ \hline
Revert           & \multicolumn{1}{c|}{\tiny\faCircle}                                                        &                                                                                                       &                                                                            \\ \hline
Out-of-gas       & \multicolumn{1}{c|}{\tiny\faCircle}                                                        &                                                                                                       &                                                                            \\ \hline
Correctness      &                                                                               & \multicolumn{1}{c|}{\tiny\faCircle}                                                                                &                                                                            \\ \hline
Integrity        &                                                                               & \multicolumn{1}{c|}{\tiny\faCircle}                                                                                & \multicolumn{1}{c|}{\tiny\faCircle}                                                     \\ \hline
Latent integrity &                                                                               &                                                                                                       & \multicolumn{1}{c|}{\tiny\faCircle}                                                     \\ \hline
\end{tabular}
\end{table}

==> tables/mappingOdc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[h]
\tiny
\centering
\caption{Mapping of our fault model to the defects detected by the tools.}
\label{tab:odc_vs_tools}
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Fault}  & \textbf{Securify}                         & \textbf{Slither}                             & \textbf{Mythril} \\ \hline
A\_MC           & CallToDefaultConstructor?                 & void-cst                                     & SWC-118          \\ \hline
A\_MCV          & -                                         & -                                            & SWC-102          \\ \hline
A\_MILV         & {\color[HTML]{24292F} UninitializedLocal} & {\color[HTML]{24292F} uninitialized-local}   & SWC-109          \\ \hline
A\_MISP         & UninitializedStorage                      & {\color[HTML]{24292F} uninitialized-storage} & SWC-109          \\ \hline
A\_MISV         & UninitializedStateVariable                & uninitialized-state                          & SWC-109          \\ \hline
A\_WCN          & CallToDefaultConstructor?                 & void-cst                                     & SWC-118          \\ \hline
A\_WDISV        & {\color[HTML]{24292F} ConstableStates}    & constable-states                             & -                \\ \hline
A\_WIS          & -                                         & storage-array                                & SWC-101          \\ \hline
A\_MIT          & -                                         & divide-before-multiply                       & SWC-101          \\ \hline
A\_WVAA         & -                                         & {\color[HTML]{24292F} missing-zero-check}    & -                \\ \hline
A\_WVAE         & -                                         & -                                            & -                \\ \hline
A\_WVATMD       & {\color[HTML]{24292F} TooManyDigits}      & {\color[HTML]{24292F} too-many-digits}       & SWC-101          \\ \hline
A\_WVN          & ShadowedStateVariable                     & shadowing-state                              & SWC-119          \\ \hline
A\_WVT          & -                                         & controlled-array-length                      & -                \\ \hline
AL\_ECSWS       & CallInLoop                                & calls-loop                                   & SWC-104          \\ \hline
AL\_MIIVS       & -                                         & -                                            & SWC-123          \\ \hline
AL\_MITSS       & UnrestrictedEtherFlow                     & unchecked-send                               & SWC-105          \\ \hline
AL\_WEH         & UnhandledException                        & unchecked-lowlevel                           & -                \\ \hline
AL\_WRAR        & -                                         & {\color[HTML]{24292F} assert-state-change}   & SWC-110          \\ \hline
CH\_MCHAO       & -                                         & -                                            & SWC-123          \\ \hline
CH\_MCHGL       & -                                         & {\color[HTML]{24292F} costly-loop}           & SWC-128          \\ \hline
CH\_MCHSF       & UnrestrictedSelfdestruct                  & suicidal                                     & SWC-106          \\ \hline
CH\_MRAIV       & -                                         & -                                            & SWC-123          \\ \hline
CH\_MRATS       & -                                         & -                                            & SWC-123          \\ \hline
CH\_MRIV        & -                                         & -                                            & SWC-123          \\ \hline
CH\_MROIV       & -                                         & -                                            & SWC-123          \\ \hline
CH\_MROTS       & -                                         & -                                            & SWC-123          \\ \hline
CH\_MRTS        & -                                         & -                                            & SWC-123          \\ \hline
CH\_WRA         & TxOrigin                                  & tx-origin                                    & SWC-115          \\ \hline
F\_EINHERITANCE & -                                         & missing-inheritance                          & SWC-125          \\ \hline
F\_MINHERITANCE & -                                         & missing-inheritance                          & SWC-125          \\ \hline
F\_MWF          & LockedEther                               & locked-ether                                 & -                \\ \hline
F\_WIO          & -                                         & missing-inheritance                          & SWC-125          \\ \hline
I\_MFVM         & ExternalFunctions                         & external-function                            & -                \\ \hline
I\_MVMSV        & StateVariablesDefaultVisibility           & -                                            & SWC-108          \\ \hline
I\_WVPF         & -                                         & constant-function-asm                        & -                \\ \hline
\end{tabular}
\end{table}

==> tables/related-surveys.tex <==
\begin{table}[H]
    \centering
    \caption{Number of papers analyzed in the related reviews.}
    \label{tab:related-surveys}
    %\resizebox{\textwidth}{!}{%
        \begin{tabular}{@{\hspace{1.5mm}}lcccc|ccc@{\hspace{1.5mm}}}
            \toprule
            & Period & Total papers & Security assessment \\
            & & & of smart contracts \\
            \midrule
            Harz \& Knottenbelt, 2018 \cite{harz_towards_2018} & 2007-2018 & 36 & 17 \\
            di Angelo \& Salzer, 2019 \cite{di_angelo_survey_2019} & 2017-2018 & 34 & 29 \\
            Praitheeshan et al., 2020 \cite{praitheeshan_security_2020} & 2016-2019 & 79 & 40 \\
            Singh et al., 2019 \cite{singh_blockchain_2019} & 2015-2019 & 35 & 24 \\
            Liu \& Liu, 2019 \cite{liu_survey_2019} & 2015-2019 & 53 & 34 \\
            Chen et al., 2019 \cite{chen_survey_2019} & 2015-2019 & 82 & 25 \\
            Wang et al., 2020 \cite{wang_ethereum_2020} & 2010-2020 & 78 & 38 \\
            Almakhour et al., 2020 \cite{almakhour_verification_2020} & 2008-2019 & 78 & 37 \\
            Li et al., 2020 \cite{li_survey_2020} & 2006-2017 & 37 & 5 \\
            This work & 2016-2020 & 43 & 39 \\
            \bottomrule
        \end{tabular}%
    %}
\end{table}

==> tables/table-different-blockchain-platforms.tex <==
\begin{landscape}
    \begin{table}
        \caption{Overview of the different blockchain platforms (adapted from \cite{kuo_comparison_2019})}
        \begin{tabular}{|m{2.5cm}|m{2.5cm}|m{2.5cm}|m{2.5cm}|m{2.5cm}|m{2.5cm}|m{2.5cm}|m{2.5cm}|}
             \hline
             \textbf{Blockchain platform} & \textbf{Objective} & \textbf{Privacy features} & \textbf{Network access} & \textbf{Consensus} & \textbf{Native currency} & \textbf{Smart contract support} & \textbf{Average speed}\\
             \hline
             Bitcoin & Public transactions & Financial transactions & Permissionless, public & Proof-of-Work (Mining) & Bitcoin (BTC) & No & 3.50 transactions per second \\
             \hline
             Ethereum & Automatic digital asset management & Private transactions & Permissionless, but supports private networks & Proof-of-Stake (Casper) & Ether & Yes (Solidity) (ETH) & 5.40 transactions per second \\
             \hline
             Hyperledger Fabric & Enterprise networks & Private channels & Permissioned, private & Pluggable & N/A & Yes (Chaincode) & 2500 transactions per second \\
             \hline
        \end{tabular}
        \label{table:different-blockchain-platforms}
    \end{table}
\end{landscape}









==> tables/table-vulnerabilities.tex <==
{\tiny
\begin{longtable}{|m{2.5cm}|m{10.5cm}|m{0.5cm}|m{1.5cm}|}
    \caption{Vulnerabilities identified in the literature.} \label{table-vulnerabilities} 
    \\
         
         \hline
         \textbf{Vulnerability} & \textbf{Works} & \textbf{Total} & \textbf{Year period} \\
         \hline
         \endhead
         
         Reentrancy & Wang et al. \cite{wang_vultron_2019}, Andesta et al. \cite{andesta_testing_2020}, Chapman et al. \cite{chapman_deviant_2019}, Ghaleb and Pattabiraman \cite{ghaleb_how_2020}, Tikhomirov et al. \cite{tikhomirov_smartcheck_2018}, Argañaraz et al. \cite{arganaraz_detection_2020}, Tsankov et al. \cite{tsankov_securify_2018}, Lu et al. \cite{lu_neucheck_2019}, Feist et al. \cite{feist_slither_2019}, Luu et al. \cite{luu_making_2016}, Chinen et al. \cite{chinen_hunting_2020}, Kalra et al. \cite{kalra_zeus_2018}, Ye et al. \cite{ye_clairvoyance_2020}, Grishchenko et al. \cite{bauer_semantic_2018}, Mavridou et al. \cite{mavridou_verisolid_2019}, Mavridou and Laszka \cite{meiklejohn_designing_2018}, Liu et al. \cite{liu_reguard_2018}, Nguyen et al. \cite{nguyen_sfuzz_2020}, Ashouri \cite{ashouri_etherolic_2020}, Ashraf et al. \cite{ashraf_gasfuzzer_2020}, Jiang et al. \cite{jiang_contractfuzzer_2018}, Liao et al. \cite{liao_soliaudit_2019}, Wang et al. \cite{wang_contractward_2020}, Feng et al. \cite{feng_precise_2019}, Zhang et al. \cite{zhang_soliditycheck_2019}, Brent et al. \cite{brent_ethainter_2020}, Durieux et al. \cite{durieux_empirical_2020}, Zhang et al. \cite{zhang_framework_2020} & 28 & 2016, 2018, 2019, 2020 \\[7ex]
\hline
Timestamp dependency & Wu et al. \cite{wu_mutation_2019}, Andesta et al. \cite{andesta_testing_2020}, Ghaleb and Pattabiraman \cite{ghaleb_how_2020}, Akca et al. \cite{akca_solanalyser_2019}, Tikhomirov et al. \cite{tikhomirov_smartcheck_2018}, Zhang et al. \cite{zhang_soliditycheck_2019}, Luu et al. \cite{luu_making_2016}, Nguyen et al. \cite{nguyen_sfuzz_2020}, Zhang et al. \cite{zhang_ethploit_2020}, Ashraf et al. \cite{ashraf_gasfuzzer_2020}, Jiang et al. \cite{jiang_contractfuzzer_2018}, Wang et al. \cite{wang_contractward_2020}, Akca et al. \cite{akca_solanalyser_2019}, Feng et al. \cite{feng_precise_2019}, Grishchenko et al. \cite{bauer_semantic_2018}, Argañaraz et al. \cite{arganaraz_detection_2020}, Liao et al. \cite{liao_soliaudit_2019}, Wu et al. \cite{wu_mutation_2019}, Grishchenko et al. \cite{bauer_semantic_2018}, Mavridou and Laszka \cite{meiklejohn_designing_2018}, Durieux et al. \cite{durieux_empirical_2020} & 21 & 2016, 2018, 2019, 2020 \\ [5ex]
\hline
Integer overflow and underflow & Wang et al. \cite{wang_vultron_2019}, Ghaleb and Pattabiraman \cite{ghaleb_how_2020}, Akca et al. \cite{akca_solanalyser_2019}, Lu et al. \cite{lu_neucheck_2019}, Kalra et al. \cite{kalra_zeus_2018}, \cite{ayoade_smart_2019}, Nguyen et al. \cite{nguyen_sfuzz_2020}, Ashouri \cite{ashouri_etherolic_2020}, Wang et al. \cite{wang_contractward_2020}, Akca et al. \cite{akca_solanalyser_2019}, So et al. \cite{so_verismart_2020}, Tikhomirov et al. \cite{tikhomirov_smartcheck_2018}, Andesta et al. \cite{andesta_testing_2020}, Feng et al. \cite{feng_precise_2019}, Argañaraz et al. \cite{arganaraz_detection_2020}, Liao et al. \cite{liao_soliaudit_2019}, Durieux et al. \cite{durieux_empirical_2020}, Zhang et al. \cite{zhang_framework_2020} & 18 & 2018, 2019, 2020 \\ [4ex]
\hline
Mishandled exceptions & Wang et al. \cite{wang_vultron_2019}, Wu et al. \cite{wu_mutation_2019}, Chapman et al. \cite{chapman_deviant_2019}, Ghaleb and Pattabiraman \cite{ghaleb_how_2020}, Tsankov et al. \cite{tsankov_securify_2018}, Luu et al. \cite{luu_making_2016}, Grishchenko et al. \cite{bauer_semantic_2018}, Nguyen et al. \cite{nguyen_sfuzz_2020}, Ashouri \cite{ashouri_etherolic_2020}, Jiang et al. \cite{jiang_contractfuzzer_2018}, Zhang et al. \cite{zhang_soliditycheck_2019}, Ashraf et al. \cite{ashraf_gasfuzzer_2020}, Zhang et al. \cite{zhang_framework_2020} & 13 & 2016, 2018, 2019, 2020 \\ [4ex]
\hline
Locked Ether & Argañaraz et al. \cite{arganaraz_detection_2020}, Zhang et al. \cite{zhang_soliditycheck_2019}, Tsankov et al. \cite{tsankov_securify_2018}, Feist et al. \cite{feist_slither_2019}, Nguyen et al. \cite{nguyen_sfuzz_2020}, Ashouri \cite{ashouri_etherolic_2020}, Ashraf et al. \cite{ashraf_gasfuzzer_2020}, Jiang et al. \cite{jiang_contractfuzzer_2018}, Tikhomirov et al. \cite{tikhomirov_smartcheck_2018}, Lu et al. \cite{lu_neucheck_2019}, Zhang et al. \cite{zhang_framework_2020} & 11 & 2018, 2019, 2020 \\[3ex]
\hline
Use of tx.origin & Wu et al. \cite{wu_mutation_2019}, Ghaleb and Pattabiraman \cite{ghaleb_how_2020}, Akca et al. \cite{akca_solanalyser_2019}, Tikhomirov et al. \cite{tikhomirov_smartcheck_2018}, Zhang et al. \cite{zhang_soliditycheck_2019}, Lu et al. \cite{lu_neucheck_2019}, Akca et al. \cite{akca_solanalyser_2019}, Argañaraz et al. \cite{arganaraz_detection_2020}, Kalra et al. \cite{kalra_zeus_2018}, Durieux et al. \cite{durieux_empirical_2020}, Zhang et al. \cite{zhang_framework_2020} & 11 & 2018, 2019, 2020 \\[3ex]
\hline
Gasless send (use of send instead of transfer) & Wang et al. \cite{wang_vultron_2019}, Chapman et al. \cite{chapman_deviant_2019}, Argañaraz et al. \cite{arganaraz_detection_2020}, Chang et al. \cite{chang_scompile_2019}, Nguyen et al. \cite{nguyen_sfuzz_2020}, Ashraf et al. \cite{ashraf_gasfuzzer_2020}, Jiang et al. \cite{jiang_contractfuzzer_2018}, Feng et al. \cite{feng_precise_2019}, Tikhomirov et al. \cite{tikhomirov_smartcheck_2018}, Zhang et al. \cite{zhang_framework_2020} & 10 & 2018, 2019, 2020 \\[3ex]
\hline
DoS by external contract & Mavridou et al. \cite{mavridou_verisolid_2019}, Tikhomirov et al. \cite{tikhomirov_smartcheck_2018}, Zhang et al. \cite{zhang_soliditycheck_2019}, Ghaleb and Pattabiraman \cite{ghaleb_how_2020}, Lu et al. \cite{lu_neucheck_2019}, Liao et al. \cite{liao_soliaudit_2019}, Ashouri \cite{ashouri_etherolic_2020}, Argañaraz et al. \cite{arganaraz_detection_2020}, Durieux et al. \cite{durieux_empirical_2020}, Zhang et al. \cite{zhang_framework_2020} & 10 & 2018, 2019, 2020 \\[3ex]
\hline
Transaction-ordering dependency (Front running) & Ghaleb and Pattabiraman \cite{ghaleb_how_2020}, Luu et al. \cite{luu_making_2016}, Mavridou and Laszka \cite{meiklejohn_designing_2018}, Liao et al. \cite{liao_soliaudit_2019}, Wang et al. \cite{wang_contractward_2020}, Kalra et al. \cite{kalra_zeus_2018}, Grishchenko et al. \cite{bauer_semantic_2018}, Tsankov et al. \cite{tsankov_securify_2018}, Durieux et al. \cite{durieux_empirical_2020}, Zhang et al. \cite{zhang_framework_2020} & 10 & 2016, 2018, 2019, 2020 \\[3ex]
\hline
DoS by block gas limit & Liao et al. \cite{liao_soliaudit_2019}, Andesta et al. \cite{andesta_testing_2020}, Akca et al. \cite{akca_solanalyser_2019}, Ashouri \cite{ashouri_etherolic_2020}, Grech et al. \cite{grech_madmax_2020}, Durieux et al. \cite{durieux_empirical_2020}, Zhang et al. \cite{zhang_framework_2020} & 7 & 2019, 2020 \\[3ex]
\hline
Unchecked low-level call functions & Tikhomirov et al. \cite{tikhomirov_smartcheck_2018}, Liao et al. \cite{liao_soliaudit_2019}, Feng et al. \cite{feng_precise_2019}, Andesta et al. \cite{andesta_testing_2020}, Argañaraz et al. \cite{arganaraz_detection_2020}, Durieux et al. \cite{durieux_empirical_2020}, Zhang et al. \cite{zhang_framework_2020} & 7 & 2018, 2019, 2020 \\[3ex]
\hline
Vulnerable Access Control & Hartel and Schumi \cite{hartel_mutation_2020}, Lu et al. \cite{lu_neucheck_2019}, Mavridou and Laszka \cite{meiklejohn_designing_2018}, Zhang et al. \cite{zhang_ethploit_2020}, Liao et al. \cite{liao_soliaudit_2019}, Feng et al. \cite{feng_precise_2019} & 6 & 2018, 2019, 2020 \\[3ex]
\hline
Unchecked delegatecall function (a type of low-level call function) & Ashraf et al. \cite{ashraf_gasfuzzer_2020}, Jiang et al. \cite{jiang_contractfuzzer_2018}, Wu et al. \cite{wu_mutation_2019}, Andesta et al. \cite{andesta_testing_2020}, Nguyen et al. \cite{nguyen_sfuzz_2020}, Brent et al. \cite{brent_ethainter_2020} & 6 & 2018, 2019, 2020 \\
\hline
Unchecked send function / Lost ether (a type of low-level call function) & Ghaleb and Pattabiraman \cite{ghaleb_how_2020}, Akca et al. \cite{akca_solanalyser_2019}, Lu et al. \cite{lu_neucheck_2019}, Kalra et al. \cite{kalra_zeus_2018}, Chapman et al. \cite{chapman_deviant_2019}, Tsankov et al. \cite{tsankov_securify_2018} & 6 & 2018, 2019, 2020 \\
\hline
Short Address Attack & Chang et al. \cite{chang_scompile_2019}, Ashouri \cite{ashouri_etherolic_2020}, Liao et al. \cite{liao_soliaudit_2019}, Feng et al. \cite{feng_precise_2019}, Durieux et al. \cite{durieux_empirical_2020}, Zhang et al. \cite{zhang_framework_2020} & 6 & 2019, 2020 \\ [1ex]
\hline
Suicidal contracts & Feist et al. \cite{feist_slither_2019}, Chang et al. \cite{chang_scompile_2019}, Krupp and Rossow \cite{krupp_teether_2018}, Brent et al. \cite{brent_ethainter_2020}, Durieux et al. \cite{durieux_empirical_2020}, Zhang et al. \cite{zhang_framework_2020} & 6 & 2018, 2019, 2020 \\ [1ex]
\hline
Out of Gas Exception & Chapman et al. \cite{chapman_deviant_2019}, Akca et al. \cite{akca_solanalyser_2019}, Tikhomirov et al. \cite{tikhomirov_smartcheck_2018}, Argañaraz et al. \cite{arganaraz_detection_2020}, Grech et al. \cite{grech_madmax_2020} & 5 & 2018, 2019, 2020 \\ [1ex]
\hline
Default visibility & Wu et al. \cite{wu_mutation_2019}, Tikhomirov et al. \cite{tikhomirov_smartcheck_2018}, Zhang et al. \cite{zhang_soliditycheck_2019}, Lu et al. \cite{lu_neucheck_2019}, Zhang et al. \cite{zhang_framework_2020} & 5 & 2018, 2019, 2020 \\ [1ex]
\hline
Bad randomness & Grishchenko et al. \cite{bauer_semantic_2018}, Ashouri \cite{ashouri_etherolic_2020}, Liao et al. \cite{liao_soliaudit_2019}, Feng et al. \cite{feng_precise_2019}, Durieux et al. \cite{durieux_empirical_2020} & 5 & 2018, 2019, 2020 \\ [1ex]
\hline
Unsafe type inference & Tikhomirov et al. \cite{tikhomirov_smartcheck_2018}, Argañaraz et al. \cite{arganaraz_detection_2020}, Zhang et al. \cite{zhang_soliditycheck_2019}, Lu et al. \cite{lu_neucheck_2019}, Torres et al. \cite{torres_osiris_2018} & 5 & 2018, 2019, 2020 \\[1ex]
\hline
Arbitrary sending of Ether & Feist et al. \cite{feist_slither_2019}, Chang et al. \cite{chang_scompile_2019}, Krupp and Rossow \cite{krupp_teether_2018}, Zhang et al. \cite{zhang_framework_2020} & 4 & 2018, 2019, 2020 \\
\hline
Constructor name & Andesta et al. \cite{andesta_testing_2020}, Zhang et al. \cite{zhang_soliditycheck_2019}, Brent et al. \cite{brent_ethainter_2020}, Zhang et al. \cite{zhang_framework_2020} & 4 & 2019, 2020 \\[1ex]
\hline
Integer division & Argañaraz et al. \cite{arganaraz_detection_2020}, Tikhomirov et al. \cite{tikhomirov_smartcheck_2018}, Zhang et al. \cite{zhang_soliditycheck_2019}, Zhang et al. \cite{zhang_framework_2020} & 4 & 2018, 2019, 2020 \\[1ex]
\hline
Unknown libraries & Andesta et al. \cite{andesta_testing_2020}, Tikhomirov et al. \cite{tikhomirov_smartcheck_2018}, Lu et al. \cite{lu_neucheck_2019}, Argañaraz et al. \cite{arganaraz_detection_2020} & 4 & 2018, 2019, 2020 \\[1ex]
\hline
Unfixed compiler version & Tikhomirov et al. \cite{tikhomirov_smartcheck_2018}, Zhang et al. \cite{zhang_soliditycheck_2019}, Lu et al. \cite{lu_neucheck_2019}, Zhang et al. \cite{zhang_framework_2020} & 4 & 2018, 2019, 2020 \\
\hline
Use of byte[ ] & Tikhomirov et al. \cite{tikhomirov_smartcheck_2018}, Zhang et al. \cite{zhang_soliditycheck_2019}, Lu et al. \cite{lu_neucheck_2019}, Zhang et al. \cite{zhang_framework_2020} & 4 & 2018, 2019, 2020 \\[1ex]
\hline
Token API violation & Tikhomirov et al. \cite{tikhomirov_smartcheck_2018}, Zhang et al. \cite{zhang_soliditycheck_2019}, Lu et al. \cite{lu_neucheck_2019}, Zhang et al. \cite{zhang_framework_2020} & 4 & 2018, 2019, 2020 \\[1ex]
\hline
Unstandardized naming & Tikhomirov et al. \cite{tikhomirov_smartcheck_2018}, Zhang et al. \cite{zhang_soliditycheck_2019}, Lu et al. \cite{lu_neucheck_2019}, Zhang et al. \cite{zhang_framework_2020} & 4 & 2018, 2019, 2020 \\
\hline
Costly loop & Tikhomirov et al. \cite{tikhomirov_smartcheck_2018}, Zhang et al. \cite{zhang_soliditycheck_2019}, Lu et al. \cite{lu_neucheck_2019}, Zhang et al. \cite{zhang_framework_2020} & 4 & 2018, 2019, 2020 \\[1ex]
\hline
Integer overflow & Gao et al. \cite{gao_easyflow_2019}, Zhang et al. \cite{zhang_soliditycheck_2019}, Grech et al. \cite{grech_madmax_2020} & 3 & 2019, 2020 \\[1ex]
\hline
Division by zero & Akca et al. \cite{akca_solanalyser_2019}, So et al. \cite{so_verismart_2020}, Torres et al. \cite{torres_osiris_2018} & 3 & 2018, 2019 \\[1ex]
\hline
Uninitialized variables & Wu et al. \cite{wu_mutation_2019}, Feist et al. \cite{feist_slither_2019}, Zhang et al. \cite{zhang_framework_2020} & 3 & 2019, 2020 \\[1ex]
\hline
Strict Balance equality & Tikhomirov et al. \cite{tikhomirov_smartcheck_2018}, Argañaraz et al. \cite{arganaraz_detection_2020}, Lu et al. \cite{lu_neucheck_2019} & 3 & 2018, 2019, 2020 \\[1ex]
\hline
Private modifier & Tikhomirov et al. \cite{tikhomirov_smartcheck_2018}, Zhang et al. \cite{zhang_soliditycheck_2019}, Lu et al. \cite{lu_neucheck_2019} & 3 & 2018, 2019 \\[1ex]
\hline
Unnecessary payable fallback function & Tikhomirov et al. \cite{tikhomirov_smartcheck_2018}, Zhang et al. \cite{zhang_soliditycheck_2019}, Lu et al. \cite{lu_neucheck_2019} & 3 & 2018, 2019 \\
\hline
Variables that should be declared as constants & Feist et al. \cite{feist_slither_2019}, Zhang et al. \cite{zhang_framework_2020} & 2 & 2019, 2020 \\
\hline
Functions that should be declared as externals & Feist et al. \cite{feist_slither_2019}, Zhang et al. \cite{zhang_framework_2020} & 2 & 2019, 2020 \\
\hline
BatchOverflow & Feng et al. \cite{feng_precise_2019}, Wu et al. \cite{wu_mutation_2019} & 2 & 2019 \\[1ex]
\hline
Integer truncation & Torres et al. \cite{torres_osiris_2018}, Zhang et al. \cite{zhang_framework_2020} & 2 & 2018, 2020 \\[1ex]
\hline
Call to the unknown & Chapman et al. \cite{chapman_deviant_2019}, Grishchenko et al. \cite{bauer_semantic_2018} & 2 & 2018, 2019 \\[1ex]
\hline
Hash collision & Lu et al. \cite{lu_neucheck_2019}, Zhang et al. \cite{zhang_framework_2020} & 2 & 2019, 2020 \\[1ex]
\hline
Shadow Memory & Feist et al. \cite{feist_slither_2019}, Ashouri \cite{ashouri_etherolic_2020} & 2 & 2019, 2020 \\[1ex]
\hline
Exposed secret & Zhang et al. \cite{zhang_ethploit_2020}, Zhang et al. \cite{zhang_framework_2020} & 2 & 2020 \\[1ex]
\hline
Callstack depth attack & Wang et al. \cite{wang_contractward_2020} & 1 & 2020 \\[1ex]
\hline
Block state dependency  (is a type of Bad randomness) & Kalra et al. \cite{kalra_zeus_2018} & 1 & 2018 \\
\hline
Race condition & Ashouri \cite{ashouri_etherolic_2020} & 1 & 2020 \\[1ex]
\hline
Repetitive contract code and clone-related bugs & Gao et al. \cite{gao_smartembed_2019} & 1 & 2019 \\
\hline
Type casts & Chapman et al. \cite{chapman_deviant_2019} & 1 & 2019 \\[1ex]
\hline
Dependence on predictable variables & Lu et al. \cite{lu_neucheck_2019} & 1 & 2019 \\[1ex]
\hline
Use of fixed-point number type & Zhang et al. \cite{zhang_soliditycheck_2019} & 1 & 2019 \\
\hline
Event-ordering (EO) bugs & Kolluri et al. \cite{kolluri_exploiting_2019} & 1 & 2019 \\
\hline
Unchecked transfer value & Zhang et al. \cite{zhang_ethploit_2020}  & 1 & 2020 \\[1ex]
\hline
Unsolvable constraints & Zhang et al. \cite{zhang_ethploit_2020} & 1 & 2020 \\[1ex]
         \hline
    \end{longtable}
    }

==> tables/table1-revocationMechanisms.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[htbp]
\caption{Revocation Approaches}
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Mechanism} & \textbf{Features}                                                                                                                                                                                                              & \textbf{Limitations}                                                                                                                                                                                                         & \textbf{Application}                                                         & \textbf{References}                                                                                                                                                                                                                                                     \\ \hline
Redacting          & \begin{tabular}[c]{@{}l@{}}a) Enables the private key holder \\ to change any block\\ b) Modifies the consensus mechanism\end{tabular}                                                                                         & \begin{tabular}[c]{@{}l@{}}a) It is not compatible with the \\ current blockchain architecture\\ b) Chameleon hashes have the \\ key exposure problem\\ c) Weaken security guarantee \\ for transactions directly \\ referencing redacted data

\end{tabular}                            & Data maintenance                                                             & \begin{tabular}[c]{@{}l@{}}Grigoriev 2021 \cite{Grigoriev2021}\\ Ateniese et al. 2017  \cite{Ateniese2017a}\\ Deuber  et al. 2019 \cite{Deuber2019}\end{tabular}                                                     \\ \hline
Pruning            & \begin{tabular}[c]{@{}l@{}}a) Reduces network size\\ b) Creates an extension of the block \\ validation algorithm\end{tabular}                                                                                                 & \begin{tabular}[c]{@{}l@{}}a) It is not compatible with the \\ current blockchain architecture\\ b) Removal occurs only on \\ local copies\\ c) Old copies of the blockchain \\ keeps the unchanged information\end{tabular} & Data maintenance                                                             & \begin{tabular}[c]{@{}l@{}}Matzutt et al. 2020 \cite{9142720}\\ Chepurnoy et al. 2016\\ Reddy 2021 \cite{Reddy2021}\end{tabular}                                                                                                      \\ \hline
Erasing            & \begin{tabular}[c]{@{}l@{}}a) Allows data removal in a local \\ blockchain\\ b) Compatible with GDPR\\ c) Allows removing partially data \\ from the block\end{tabular}                                                              & \begin{tabular}[c]{@{}l@{}}a) It is not compatible with the \\ current blockchain architecture\\ b) Non-scalable, mainly for \\ public networks\end{tabular}                                                                 & Data maintenance                                                             & \begin{tabular}[c]{@{}l@{}}Florian et al. 2019 \cite{Florian2019}\\ Kuhn 2020 \cite{Kuhn2020}\end{tabular}                                                                                                                            \\ \hline
Accumulators       & \begin{tabular}[c]{@{}l@{}}a) Allows backward compatibility\\ with PKI system\\ b) Implements new transactions models\\  to store revoked records\\ c) Uses cryptographic accumulators\\ to store revoked records\end{tabular} & \begin{tabular}[c]{@{}l@{}}a) Costs are unpredictable\\ b) Limited storage of \\ information\end{tabular}                                                                                                                       & \begin{tabular}[c]{@{}l@{}}Authentication\\ Asset inactivation\end{tabular} & \begin{tabular}[c]{@{}l@{}}Wang et al. 2019 \cite{Wang2019}\\ Yu et al. 2020 \cite{Yu2020}\end{tabular}                                                                                                                               \\ \hline
List               & \begin{tabular}[c]{@{}l@{}}a) Improves the revocation mechanism \\ compared to the RSA system\\ b) Allows revoking multiple records with\\ low costs\end{tabular}                                                              & \begin{tabular}[c]{@{}l@{}}a) Easy to tamper\\ b) Centralized system\end{tabular}                                                                                                                                            & \begin{tabular}[c]{@{}l@{}}Authentication\\ Asset inactivation\end{tabular} & \begin{tabular}[c]{@{}l@{}}MIT Lab 2016 \cite{M.L.MITMediaLab2016}\\ Ronning 2019 \cite{Ronning2019}\end{tabular}                                                                                                                     \\ \hline
Forking          & \begin{tabular}[c]{@{}l@{}}a) Creates a new network isolating\\ the revoked records\\ b) Keeps the existence of the old data\end{tabular}                                                                                      & \begin{tabular}[c]{@{}l@{}}a) It is not feasible for\\ small operations\\ b) Demands off-chain consensus\end{tabular}                                                                                                        & Data maintenance                                                             & Siegel 2016 \cite{Siegel2016}                                                                                                                                                                                                                          \\ \hline
Preventing           & \begin{tabular}[c]{@{}l@{}}a) Uses content detectors based\\ on heuristics mechanisms\\ b) It is compatible with any blockchain\end{tabular}                                                                                   & \begin{tabular}[c]{@{}l@{}}a) Limited scope action, is not \\ possible to  avoid recording any \\ unwanted data.\end{tabular}                                                                                                    & Prevents harmful data                                                        & Matzutt et al. 2018 \cite{Matzutt2018}                                                                                                                                                                                                                 \\ \hline
Smart contracts    & \begin{tabular}[c]{@{}l@{}}a) Creates states based on smart contracts \\ to refer a record valid or revoked\end{tabular}                                                                                                       & \begin{tabular}[c]{@{}l@{}}a) Non-agnostic blockchain\\ b) The trust of the revocation\\ status relies on software \\ build arbitrarily\end{tabular}                                                                            & \begin{tabular}[c]{@{}l@{}}Authentication\\ Asset inactivation\end{tabular} & \begin{tabular}[c]{@{}l@{}}Hewa 2020 et al. \cite{Hewa2020}\\ Hu 2020 \cite{Hu2020}\\ Kubilay et al. 2018 \cite{DBLP:journals/corr/abs-1806-03914}\\ Reen et. al. 2019 \cite{Reen2019}\end{tabular} \\ \hline
\end{tabular}
\label{Tabela1}
\end{table*}

==> tables/table2-mechanismsAnalysis.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htbp]
\caption{Mechanism application analysis}
\begin{tabular}{|l|l|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Mechanism}}}                  & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{References}}}                                                & \multicolumn{2}{c|}{\textbf{Blockchain Compatibility}}                                                              & \multicolumn{2}{c|}{\textbf{Network Target}}               & \multicolumn{4}{c|}{\textbf{Consensus Changing}}                                                                                                           & \multicolumn{3}{c|}{\textbf{Reported Security Analysis}}                                                                                                                                                                                                      \\ \cline{3-13} 
\multicolumn{1}{|c|}{}                                                     & \multicolumn{1}{c|}{}                                                                                    & \multicolumn{1}{l|}{New Design} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Current \\ System(s)\end{tabular}} & \multicolumn{1}{l|}{Public} & \multicolumn{1}{l|}{Private} & \multicolumn{1}{l|}{PoW} & \multicolumn{1}{l|}{BFT} & \multicolumn{1}{l|}{PA} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}New \\ Design\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Pri-\\ vacy\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Attacks\\ DOS\\ 51\%\\ Double \\ spend\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Perfor-\\ mance\end{tabular}} \\ \hline
\multirow{3}{*}{Redacting}                                                 & \begin{tabular}[c]{@{}l@{}}Ateniese et al.\\ 2017 \cite{Ateniese2017a}\end{tabular}     & Bitcoin-based                   & -                                                                                 & \textbf{X}                  & -                            & \textbf{X}               & -                        & -                       & -                                                                          & \textbf{X}                                                               & -                                                                                                   & \textbf{X}                                                                   \\ \cline{2-13} 
                                                                           & \begin{tabular}[c]{@{}l@{}}Deuber et al.\\ 2019\cite{Deuber2019}\end{tabular}           & Bitcoin-based                   & -                                                                                 & \textbf{X}                  & -                            & \textbf{X}               & -                        & -                       & -                                                                          & -                                                                        & \textbf{X}                                                                                          & \textbf{X}                                                                   \\ \cline{2-13} 
                                                                           & \begin{tabular}[c]{@{}l@{}}Grigoriev \\2021 \cite{Grigoriev2021}\end{tabular}           & Agnostic                        & -                                                                                 & -                           & \textbf{X}                   & -                        & -                        & -                       & \textbf{X}                                                                 & -                                                                        & -                                                                                                   & -                                                                            \\ \hline
\multirow{3}{*}{Pruning}                                                   & \begin{tabular}[c]{@{}l@{}}Chepurnoy et al.\\ 2016\cite{Chepurnoy2016}\end{tabular}     & Bitcoin-based                   & -                                                                                 & \textbf{X}                  & -                            & \textbf{X}               & -                        & -                       & -                                                                          & -                                                                        & \textbf{X}                                                                                          & -                                                                            \\ \cline{2-13} 
                                                                           & \begin{tabular}[c]{@{}l@{}}Reddy \\ 2021 \cite{Reddy2021}\end{tabular}                   & Bitcoin-based                   & -                                                                                 & \textbf{X}                  & -                            & \textbf{X}               & -                        & -                       & -                                                                          & -                                                                        & \textbf{X}                                                                                          & -                                                                            \\ \cline{2-13} 
                                                                           & \begin{tabular}[c]{@{}l@{}}Matzutt et al.\\ 2020 \cite{9142720}\end{tabular}             & -                               & \begin{tabular}[c]{@{}c@{}}Bitcoin via \\ velvet fork\end{tabular}                & \textbf{X}                  & -                            & -                        & -                        & -                       & \textbf{X}                                                                 & -                                                                        & \textbf{X}                                                                                          & \textbf{X}                                                                   \\ \hline
\multirow{2}{*}{Erasing}                                                   & \begin{tabular}[c]{@{}l@{}}Florian et al.\\2019 \cite{Florian2019}\end{tabular}         & -                               & \begin{tabular}[c]{@{}c@{}}Bitcoin \\ local copy\end{tabular}                     & -                           & \textbf{X}                   & -                        & -                        & -                       & \textbf{X}                                                                 & -                                                                        & -                                                                                                   & -                                                                            \\ \cline{2-13} 
                                                                           & \begin{tabular}[c]{@{}l@{}}Kuhn 2020\\ \cite{Kuhn2020}\end{tabular}                       & Matrix Block                    & -                                                                                 & -                           & \textbf{X}                   & -                        & -                        & -                       & \textbf{X}                                                                 & -                                                                        & -                                                                                                   & -                                                                            \\ \hline
\multirow{2}{*}{Accumulators}                                              & \begin{tabular}[c]{@{}l@{}}Karasavvas \\2018 \cite{Karasavvas2018}\end{tabular}         & -                               & Bitcoin                                                                           & \textbf{X}                  & -                            & -                        & -                        & -                       & -                                                                          & -                                                                        & -                                                                                                   & -                                                                            \\ \cline{2-13} 
                                                                           & \begin{tabular}[c]{@{}l@{}}Khovratovich \\2016 \cite{Khovratovich2016}\end{tabular}     & -                               & Sovrin                                                                            & \textbf{X}                  & \textbf{X}                   & -                        & \textbf{X}               & -                       & -                                                                          & \textbf{X}                                                               & -                                                                                                   & \textbf{X}                                                                   \\ \hline
\multirow{2}{*}{List}                                                      & \begin{tabular}[c]{@{}l@{}}Vidal et al.\\2020 \cite{ASTESJ2020}\end{tabular}            & -                               & \begin{tabular}[c]{@{}c@{}}Ethereum\\ Bitcoin\end{tabular}                        & \textbf{X}                  & \textbf{X}                   & -                        & -                        & -                       & -                                                                          & \textbf{X}                                                               & -                                                                                                   & -                                                                            \\ \cline{2-13} 
                                                                           & \begin{tabular}[c]{@{}l@{}}Ronning \\2019 \cite{Ronning2019}\end{tabular}               & -                               & \begin{tabular}[c]{@{}c@{}}Ethereum\\ Bitcoin\end{tabular}                        & \textbf{X}                  & \textbf{X}                   & -                        & -                        & -                       & -                                                                          & \textbf{X}                                                               & -                                                                                                   & -                                                                            \\ \hline
\multirow{2}{*}{Forking}                                                   & \begin{tabular}[c]{@{}l@{}}Javarone \\2018 \cite{Javarone2018}\end{tabular}             & -                               & Bitcoin Cash                                                                      & \textbf{X}                  & -                            & -                        & -                        & -                       & -                                                                          & -                                                                        & \textbf{X}                                                                                          & -                                                                            \\ \cline{2-13} 
                                                                           & \begin{tabular}[c]{@{}l@{}}Hanke \\2016  \cite{DBLP:journals/corr/Hanke16}\end{tabular} & -                               & Bitcoin Gold                                                                      & \textbf{X}                  & -                            & -                        & -                        & -                       & -                                                                          & -                                                                        & \textbf{X}                                                                                          & -                                                                            \\ \hline
Preventing                                                                   & \begin{tabular}[c]{@{}l@{}}Matzutt et al.\\ 2018 \cite{Matzutt2018}\end{tabular}        & -                               & Bitcoin                                                                           & \textbf{X}                  & -                            & -                        & -                        & -                       & -                                                                          & -                                                                        & -                                                                                                   & -                                                                            \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Smart \\ Contract\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Hewa et al.\\2020  \cite{Hewa2020}\end{tabular}              & -                               & Hyperledger                                                                       & -                           & \textbf{X}                   & -                        & \textbf{X}               & -                       & -                                                                          & -                                                                        & -                                                                                                   & \textbf{X}                                                                   \\ \cline{2-13} 
                                                                           & \begin{tabular}[c]{@{}l@{}}Reen et al.\\2019 \cite{Reen2019}\end{tabular}               & -                               & Ethereum                                                                          & \textbf{-}                  & \textbf{X}                   & -                        & -                        & \textbf{X}              & -                                                                          & \textbf{X}                                                               & -                                                                                                   & -                                                                            \\ \hline
\end{tabular}
\label{Tabela2}
\end{table*}
